Is Conversational XAI All You Need? Human-AI Decision Making With a Conversational XAI Assistant

Explainable artificial intelligence (XAI) methods are being proposed to help interpret and understand how AI systems reach specific predictions. Inspired by prior work on conversational user interfaces, we argue that augmenting existing XAI methods with conversational user interfaces can increase user engagement and boost user understanding of the AI system. In this paper, we explored the impact of a conversational XAI interface on users' understanding of the AI system, their trust, and reliance on the AI system. In comparison to an XAI dashboard, we found that the conversational XAI interface can bring about a better understanding of the AI system among users and higher user trust. However, users of both the XAI dashboard and conversational XAI interfaces showed clear overreliance on the AI system. Enhanced conversations powered by large language model (LLM) agents amplified over-reliance. Based on our findings, we reason that the potential cause of such overreliance is the illusion of explanatory depth that is concomitant with both XAI interfaces. Our findings have important implications for designing effective conversational XAI interfaces to facilitate appropriate reliance and improve human-AI collaboration. Code can be found at https://github.com/delftcrowd/IUI2025_ConvXAI

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/sec-result.tex <==
\section{Experimental Results}
%\ug{Will continue from here in the morning! Good night. :-)}
In this section, we present the experimental results of our empirical study. We discuss the descriptive statistics, hypotheses test results, and further exploratory findings. To test the aforementioned hypotheses, we relied on appropriate statistical analyses. In addition to such confirmatory analyses, we carried out exploratory analyses to draw nuanced interpretations of our main insights.
Our code and data can be found at the OSF repository for the benefit of the community and in the spirit of open science.\footnote{\url{https://osf.io/j8s69/?view_only=056d696cd8e648f0bab04bf0f3f6016e}}
% ~\glcomment{To check whether we should release one anonymized osf link here.}


\subsection{Descriptive Statistics}
To ensure the reliability of our results and interpretations, we only consider participants who passed all attention checks. 
Finally, the participants considered for analysis were distributed in a balanced manner across the four experimental conditions: 61 (\control{}), 61 (\dashboard{}), 62 (\chatxai{}), 61 (\chatpersonalized{}), 
\revise{61 (\chatagent{}). On average, each task consumes 13 API calls to obtain GPT-4 responses, including generating reply messages and XAI usage.}

\paratitle{Distribution of Covariates}. The covariates’ distribution is as follows: 
\textit{ML Background} ($21.6\%$ with machine learning background knowledge, $78.4\%$ without machine learning background knowledge), 
\textit{ATI} ($M = 3.97$, $SD = 0.92$; 6-point Likert scale, \textit{1: low, 6: high}), 
\textit{TiA-Propensity to Trust} ($M = 2.90$, $SD = 0.67$; 5-point Likert scale, \textit{1: tend to distrust}, \textit{5: tend to trust}), 
and \textit{TiA-Familiarity} ($M = 2.61$, $SD = 1.08$; 5-point Likert scale, \textit{1: unfamiliar}, \textit{5: very familiar}). 

\paratitle{Performance Overview}. On average across all conditions, participants achieved an accuracy of
$64.8\%$ ($SD = 0.11$), which is still lower than the AI accuracy ($70\%$). The agreement fraction is 0.836 ($SD = 0.17$), and the
switching fraction is 0.509 ($SD = 0.42$). With these measures, we confirm that when users disagree with AI advice, they do not always blindly rely on AI advice. 
As all dependent variables are not normally distributed, we used non-parametric statistical tests to verify our hypotheses.
% \glcomment{shall we provide more info about user trust?}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/explanation_utility_bar_plot.pdf}
    \caption{Bar plot illustrating the explanation utility across conditions. The error bars represent the $95\%$ confidence interval.}%glcomment{Do you think the color is too light?} \ug{Keep the error bars.}\glcomment{If you have any suggestions about error bar thickness / cap size, let me know}}
    \label{fig:explanation_utility}
    \Description{Bar plots for explanation utility (Explanation Completeness, Explanation Coherence, Explanation Clarity, and Explanation Usefulness) across conditions with XAI interfaces. Overall, all conditions achieved similar Explanation Completeness and Explanation Clarity. Meanwhile, the conversational XAI interfaces achieved slightly better Explanation Coherence and Explanation Usefulness.}
\end{figure*}

\paratitle{Explanation Utility}. To illustrate how the XAI interface will affect the perceived explanation utility, we adopted a bar plot of explanation utility across conditions (including the \chatagent{} condition in the follow-up study). As shown in Figure~\ref{fig:explanation_utility}, participants achieved similar level of \textit{Explanation Completeness} and \textit{Explanation Clarity}. Meanwhile, participants with conversational XAI interfaces (\ie condition \chatxai{}, \chatpersonalized{}, and \chatagent{}) achieved slightly higher \textit{Explanation Coherence} and \textit{Explanation Usefulness}. Based
on one-way ANOVA, we analyzed the impact of XAI interfaces in perceived explanation utility. There is no significant difference across conditions.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/explanation_utility_bar_plot.pdf}
%     \caption{Bar plot illustrating the explanation utility across conditions. The error bars represent the $95\%$ confidence interval.}%glcomment{Do you think the color is too light?} \ug{Keep the error bars.}\glcomment{If you have any suggestions about error bar thickness / cap size, let me know}}
%     \label{fig:explanation_utility}
%     \Description{Bar plots for explanation utility (Explanation Completeness, Explanation Coherence, Explanation Clarity, and Explanation Usefulness) across conditions with XAI interfaces. Overall, all conditions achieved similar Explanation Completeness and Explanation Clarity. Meanwhile, the conversational XAI interfaces achieved slightly better Explanation Coherence and Explanation Usefulness.}
% \end{figure}


% \paratitle{Usage of Different XAI methods}. 
% For participants in the condition \chatxai{} and \chatpersonalized{}, we analyzed their usage of XAI methods to understand users' information needs. 
% In our analysis, the usage frequency of the five XAI methods are: global explanation (\ie PDP, $46.5\%$ of total usage), SHAP ($24.4\%$ of total usage), WhatIf ($13.0\%$ of total usage), Decision Tree ($10.0\%$ of total usage), Counterfactual (\ie MACE, $6.1\%$ of total usage).\glcomment{It can be removed, as we elaborate on the XAI usage in further analysis} \ug{Agreed!}

%\glcomment{Clarify the goals of the statistical analysis and the importance of the result (R1).}

\subsection{Hypothesis Tests}
\label{sec-hyp-test}
%To provide a smooth reading experience and fit the page limits, 
For the convenience of the readers, we have provided concise insights in the main body of this section and placed additional tables and figures (\eg estimation plots) that provide further details in the supplementary materials. %\glcomment{separate user understanding with explanation utility, reduce the exp results length}

%\glcomment{Relatedly, revisions should clarify the goals of the statistical analysis up front and argue for the importance of the results given that the results of statistical testing could not find significant effects for many (if not most) comparisons. This is very important since some of the results towards the end seem to report excessive number of comparisons (not even including those from the appendix). With so many comparisons there is a chance that some of those significant results occurred by chance. It is unclear how the power analysis in section 4.3 accounted for so many comparisons. It is therefore important to clarify the hypotheses up front to avoid issues related to “phishing expeditions.”}

\subsubsection{\textbf{H1}: effect of XAI interfaces on user understanding}
\label{sec-h1}
% H1: Compared to the XAI dashboard, the conversational XAI interface creates a better understanding of the AI system.
% To analyze the main effect of the XAI interfaces on user understanding of the AI system, we conducted ANOVA tests by considering different experimental conditions. 
To analyze the main effect of the XAI interfaces on user understanding of the AI system, we conducted an \textit{Analysis of Covariance} (ANCOVA) with the \textit{experimental condition} as between-subjects factor and \textit{TiA-Propensity to Trust}, \textit{TiA-Familiarity}, \textit{ATI}, and \textit{ML Background} as covariates. 
While our data may not be normally distributed, we still adopted  AN(C)OVAs for analysis because these analyses have been shown to be robust to Likert-type ordinal data~\cite{Norman-2010-likert}. 
For this analysis, we considered all participants across three experimental conditions with XAI (\ie \dashboard{}, \chatxai{}, and \chatpersonalized{}).  
%The results are shown in Table~\ref{tab:H1}. 
%
% \begin{table}[htbp]
% 	\centering
% 	\caption{ANCOVA test results for \textbf{H1} on user understanding dependent variables. ``$\dagger\dagger$'' indicates the effect of the variable is significant at the level of 0.0125.
%     } 
% 	\label{tab:H1}%
% 	\begin{small}
% 	\begin{tabular}{c | c c| c c| c c| c c | c c}
% 	    \hline
% 	    \textbf{Variables}&	\multicolumn{2}{c|}{Exp Condition}& \multicolumn{2}{c|}{TiA-PtT}& \multicolumn{2}{c|}{TiA-Familiarity}& \multicolumn{2}{c|}{ATI} & \multicolumn{2}{c}{ML Background}\\
%      % \multicolumn{2}{c|}{\textbf{PFU}}& \multicolumn{2}{c|}{\textbf{Explanation Completeness}}&	\multicolumn{2}{c|}{\textbf{Explanation Coherence}}& \multicolumn{2}{c|}{\textbf{Explanation Clarity}}&	\multicolumn{2}{c|}{\textbf{Explanation Usefulness}}& \multicolumn{2}{c|}{\textbf{Learning Effect across Tasks}} & \multicolumn{3}{c}{\textbf{Understanding of System}}\\
% 	    \hline
% 	    \textbf{Dependent Variables}& $F$& $p$& $F$& $p$& $F$& $p$& $F$& $p$& $F$& $p$\\
% 	    \hline \hline
% 	    \textbf{Perceived Feature Understanding}&	1.24 & .293 & 25.80 & \textbf{.000}$^{\dagger\dagger}$ & 0.41 & .521 & 0.42 & .516 & 0.08 & .784\\
%         \textbf{Learning Effect across Tasks}& 0.42 & .658 & 9.91 & \textbf{.002}$^{\dagger\dagger}$ & 0.06 & .810 & 0.75 & .388 & 0.76 & .383\\
%         \textbf{Understanding of System}& 0.86 & .425 & 21.87 & \textbf{.000}$^{\dagger\dagger}$ & 0.60 & .441 & 10.29 & \textbf{.002}$^{\dagger\dagger}$ & 0.25 & .614\\
%         % \hline
%         % \textbf{Explanation Completeness}&	0.32 & .726 & 29.65 & \textbf{.000}$^{\dagger\dagger}$ & 2.27 & .133 & 0.33 & .564 & 2.30 & .131\\
%         % \textbf{Explanation Coherence}& 1.84 & .162 & 33.53 & \textbf{.000}$^{\dagger\dagger}$ & 0.27 & .607 & 0.71 & .401 & 0.14 & .706\\
%         % \textbf{Explanation Clarity}& 0.15 & .864 & 49.86 & \textbf{.000}$^{\dagger\dagger}$ & 3.29 & .072 & 1.31 & .254 & 0.51 & .477\\
%         % \textbf{Explanation Usefulness}& 1.18 & .310 & 44.66 & \textbf{.000}$^{\dagger\dagger}$ & 0.09 & .769 & 0.00 & .949 & 0.09 & .765\\
%         % \textbf{Learning Effect across Tasks}& 0.42 & .658 & 9.91 & \textbf{.002}$^{\dagger\dagger}$ & 0.06 & .810 & 0.75 & .388 & 0.76 & .383\\
%         % \textbf{Understanding of System}& 0.86 & .425 & 21.87 & \textbf{.000}$^{\dagger\dagger}$ & 0.60 & .441 & 10.29 & \textbf{.002}$^{\dagger\dagger}$ & 0.25 & .614\\
% 	    % \rowcolor{gray!15}TiA-Propensity to Trust&	202.23& \textbf{<.001}$^{\dagger\dagger}$& 0.45& 	61.90& \textbf{<.001}$^{\dagger\dagger}$& 0.18  &	327.91& \textbf{<.001}$^{\dagger\dagger}$& 0.57\\
% 	    % TiA-Familiarity&	2.52& .114& 0.01& 	3.39& .067& 0.01&	0.32& .574& 0.00\\
% 	    % \rowcolor{gray!15}ATI&	2.69& .103& 0.01& 	16.06& \textbf{<.001}$^{\dagger\dagger}$& 0.05&	0.63& .429& 0.00\\
% 	    % ML Background&	0.45& .503& 0.00& 0.32& .575& 0.00&	0.10& .757& 0.00\\
% 	    \hline
% 	\end{tabular}%
% 	\end{small}
% \end{table}%
%
%As shown in Table~\ref{tab:H1}, 
We found %there is 
no significant differences resulting from the %caused by the 
different XAI interfaces (\ie experimental condition). However, the \textit{TiA-Propensity to Trust} showed a significant impact on all dimensions of user understanding. Meanwhile, \textit{ATI} also shows a significant impact on the \textit{Understanding of System}. 
For the objective feature understanding (continuous value, non-normal distribution), we conducted Kruskal-Wallis H-tests by considering different XAI interfaces. No significant difference ($H = 0.07, p = .968$) was found between participants with different XAI interfaces. Thus, we did not find any support for \textbf{H1}.
% ~\glcomment{For the objective feature understanding, we found that participants in LLM Agent condition showed even significantly worse compared to other conditions. To check whether we should report this}
% ~\glcomment{For trust analysis, we used ANCOVA, but here we used ANOVA. Do we need to make them consistent?} \ug{Yes, let's do that and move the rationale for using ANCOVAs here.}
% we adopted Kruskal-Wallis H-test to compare across three conditions with XAI. 

% To further analyze the user understanding across different experimental conditions, we calculate the mean and standard deviation for each group of participants with XAI interface. 
% The results are shown in Table~\ref{tab:mean_std_h1}. 
% Participants with conversational XAI interfaces showed slightly better feedback in comparison to participants with XAI dashboard, in dimension \textit{PFU}, \textit{Explanation Coherence}, \textit{Explanation Usefulness}, and \textit{Learning Effect Across Tasks}.

% \begin{table}[htbp]
% 	\centering
% 	\caption{Mean value and standard deviation for participants with XAI interfaces. The highest value for each dependent variable is labeled with bold font.}
% 	\label{tab:mean_std_h1}%
%         % \begin{small}
%         % \scalebox{0.95}{
% 	\begin{tabular}{c | c  c  c}
% 	    \hline
%             \textbf{Dependent Variables}& $M \pm SD$ (\dashboard{})& $M \pm SD$ (\chatxai{})& $M \pm SD$ (\chatpersonalized{})\\
%             \hline
%             \hline
%             \textbf{PFU}& 4.10 $\pm$ 0.89& \textbf{4.24 $\pm$ 0.72}& 4.07 $\pm$ 0.79\\
%             % \textbf{OFU}& 0.095& .910& 0.88& \textbf{0.88}& 0.87\\
%             \textbf{Explanation Completeness}& \textbf{3.60 $\pm$ 0.67}& 3.56 $\pm$ 0.72& 3.53 $\pm$ 0.64\\
%             \textbf{Explanation Coherence}&  3.57 $\pm$ 0.97& 3.81 $\pm$ 0.92& \textbf{3.87  $\pm$ 0.99}\\
%             \textbf{Explanation Clarity}& 4.02 $\pm$ 0.83& 4.02  $\pm$ 0.76& 4.02 $\pm$ 0.83\\
%             \textbf{Explanation Usefulness}&  3.95 $\pm$ 0.75& \textbf{4.09 $\pm$ 0.67}& 4.02 $\pm$ 0.59\\
%             \textbf{Learning Effect across Tasks}&  3.93 $\pm$ 0.87& \textbf{4.06 $\pm$ 0.77}& 4.03 $\pm$ 0.73\\
%             \textbf{Understanding of System}&  \textbf{4.13 $\pm$ 0.78}& 3.95 $\pm$ 0.86& 4.03 $\pm$ 0.87\\
% 	    \hline
% 	\end{tabular}
%         % \end{small}
%     % }%
% \end{table}%

\subsubsection{\textbf{H2}: effect of XAI interfaces on user trust}
\label{sec-h2}
% H2: Compared to the XAI dashboard, the conversational XAI interface will help users exhibit a relatively higher trust in the underlying AI system.

To verify \textbf{H2} (\ie the impact of XAI interface on user trust), we conducted an 
% The impact of subjective trust was analyzed using an 
\textit{Analysis of Covariance} (ANCOVA) with the \textit{experimental condition} as between-subjects factor and \textit{TiA-Propensity to Trust}, \textit{TiA-Familiarity}, \textit{ATI}, and \textit{ML Background} as covariates. 
This allows us to explore the main effects of the XAI interface on subjective trust as measured by the three subscales of the Trust in Automation questionnaire~\cite{korber2019theoretical}. 
% We decided to conduct AN(C)OVAs despite the anticipation that 
% While our data may not be normally distributed, we still adopted AN(C)OVAs for analysis because these analyses have been shown to be robust to Likert-type ordinal data~\cite{Norman-2010-likert}. 
Table~\ref{tab:H2} shows the ANCOVA results of the three trust-related dependent variables. 
% ~\glcomment{Text copied from ANIE paper, to revise}

\begin{table*}[htbp]
	\centering
	\caption{ANCOVA test results for \textbf{H2} on trust-related dependent variables. ``$\dagger$'' and ``$\dagger\dagger$'' indicate the effect of the variable is significant at the level of 0.05 and 0.0125, respectively.
 % ~\glcomment{If we update with LLM Agent condition, we will have similar conclusions. The only difference is that the LLM Agent does not show significantly better U/P compared with Control. User trust decreased a bit on LLM Agent condition compared to other XAI interfaces.}
    % \glcomment{To think about, whether we should adopt ANOVA instead of ANCOVA. With ANOVA, we have significant results for all dimensions (in comparison with Control case).}\ug{ANCOVA results present the complete picture including the nuances of the covariates, so I would stick to the ANCOVA.}
    } 
	\label{tab:H2}%
	\begin{small}
	\begin{tabular}{c | c c c | c c c| c c c}
	    \hline
	    \textbf{Dependent Variables}&	\multicolumn{3}{c|}{\textbf{TiA-R/C}}& \multicolumn{3}{c|}{\textbf{TiA-U/P}} & \multicolumn{3}{c}{\textbf{TiA-Trust}}\\
	    \hline
	    Variables& $F$& $p$& $\eta^2$& $F$& $p$& $\eta^2$& $F$& $p$& $\eta^2$\\
	    \hline \hline
	    Exp Condition&	2.61& .052& 0.02& 6.20& \textbf{<.001}$^{\dagger\dagger}$&   0.06&	3.60& \textbf{.014}$^\dagger$& 0.02\\
	    \rowcolor{gray!15}TiA-Propensity to Trust&	202.23& \textbf{<.001}$^{\dagger\dagger}$& 0.45& 	61.90& \textbf{<.001}$^{\dagger\dagger}$& 0.18  &	327.91& \textbf{<.001}$^{\dagger\dagger}$& 0.57\\
	    TiA-Familiarity&	2.52& .114& 0.01& 	3.39& .067& 0.01&	0.32& .574& 0.00\\
	    \rowcolor{gray!15}ATI&	2.69& .103& 0.01& 	16.06& \textbf{<.001}$^{\dagger\dagger}$& 0.05&	0.63& .429& 0.00\\
	    ML Background&	0.45& .503& 0.00& 0.32& .575& 0.00&	0.10& .757& 0.00\\
	    \hline
	\end{tabular}%
	\end{small}
\end{table*}%

As can be seen, the experimental condition (\ie XAI interface) only showed a significant impact in \textbf{TiA-U/P}. 
With post-hoc Tukey's HSD test, we found that participants who received XAI showed significantly higher trust in \textbf{Understandability/Predictability} (\ie \control{} < \dashboard{}, \chatxai{}, \chatpersonalized{}). 
However, no significant difference is found between the \dashboard{} condition and conditions with conversational XAI. 
At the same time, there is no significant impact of the experimental conditions observed on the dependent variables of \textbf{TiA-R/C} and \textbf{TiA-Trust}. 
% Although non-significant differences are found for \textbf{TiA-R/C} and \textbf{TiA-Trust}, participants with conversational XAI interfaces still indicated higher trust in comparison with participants with XAI dashboard.~\glcomment{To check}
Meanwhile, we found that \textbf{TiA-Propensity to Trust} had a significant impact on all trust-related dependent variables, and that users' affinity to technology interaction (\textbf{ATI}) also had a significant impact on \textbf{TiA-U/P}.
% ~\glcomment{Increase the diversity of expression in this paragraph, too many ``we found''}

To better understand effect sizes in terms of the TiA-U/P and go beyond \textit{p}-values, we adopted an estimation plot~\cite{ho2019moving} (shown in supplementary materials, Figure 3). As reflected by the swarm plot, participants with conversational XAI interface (\ie condition \chatxai{} and \chatpersonalized{}) exhibited a marginally higher TiA-U/P in comparison with condition \dashboard{}. 
Thus, we only found partial support for \textbf{H2}.  %is partially supported by our experimental results. %~\glcomment{Can we claim it is partially supported? As it did show slightly better TiA-U/P with the estimation plot}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.5]{figures/estimation_plot_trust_understanding.png}
%     \caption{Estimation plot for TiA-U/P. The upper part shows the data point swamp plot, and the bottom part shows the sampled mean difference normal distribution in comparison to condition \control{}. 
%     % As the distribution of mean difference shows, participants in condition \chatxai{} and \chatpersonalized{} showed slightly higher TiA-U/P.
%     % \ug{Add a sentence or two to help readers understand and read the plot better.}
%     }
%     \label{fig:estimation-trust-up}
%     \Description{Estimation plot for TiA-Understandability/Predictability. From the distribution, we see that participants in condition \chatxai{} and \chatpersonalized{} showed slightly larger values.}
% \end{figure}


\subsubsection{\textbf{H3}: effect of XAI interfaces on appropriate reliance} 
\label{sec-h3}
To verify \textbf{H3}, we conducted a Kruskal-Wallis H-test to compare the performance, reliance, and appropriate reliance measures of participants across four experimental conditions. 
As shown in Table~\ref{tab:res-reliance}, participants showed significantly higher reliance (\ie \textit{Agreement Fraction} and \textit{Switch Fraction}) with access to the XAI dashboard or conversational XAI interface. 
However, the increased reliance is not necessarily appropriate reliance. 
Only participants with access to conversational XAI interface (\ie condition \chatxai{}) showed significantly better \textit{RAIR} in comparison with the condition \control{}.
We also found that participants showed significantly worse \textit{RSR} with access to the XAI dashboard or conversational XAI interface. 
There is no significant difference with respect to \textit{RAIR} or \textit{RSR} between the three conditions with access to XAI interfaces.
Thus, \textbf{H3} is not supported by our experimental results.

% H3: Compared to the XAI dashboard, the conversational XAI interface will help users exhibit a relatively more appropriate reliance on the underlying AI system.

\begin{table*}[hbpt]
% the environment \color{blue} change all cell color
	\centering
	\caption{Kruskal-Wallis H-test results for XAI interfaces (\textbf{H3} and \textbf{H4}) on reliance-based dependent variables. {The post-hoc results are based on Mann–Whitney tests.} ``${\dagger\dagger}$'' indicates the effect of the variable is significant at the level of 0.0125.
 % \glcomment{Here, we have some interesting findings after adding LLM Agent condition. We have \control{} > \dashboard{}, \chatxai{}, \chatpersonalized{}, \chatagent{} and \dashboard{}> \chatagent{} in RSR. For agreement fraction and switch fraction, with XAI interfaces > \control{}. But our improvement in RAIR becomes non-significant}
 }
	\label{tab:res-reliance}%
	\begin{small}
        \scalebox{0.95}{
	\begin{tabular}{c | c c | c c c c| c}
	    \hline
	    \multirow{2}{*}{\textbf{Dependent Variables}}& \multirow{2}{*}{$H$}& \multirow{2}{*}{$p$}& \multicolumn{4}{c|}{$M \pm SD$}& \multirow{2}{*}{Post-hoc results}\\
     \cline{4-7}
     &  & & \control& \dashboard{}& \chatxai{}& \chatpersonalized{}& \\
	    \hline \hline
	    \textbf{Accuracy}& 7.50 & .058& $0.62 \pm 0.13$ &$0.65 \pm 0.11$ &$0.67 \pm 0.10$ &$0.64 \pm 0.09$& -\\
	\rowcolor{gray!15}\textbf{Agreement Fraction}& 28.45 & \textbf{.000}$^{\dagger\dagger}$& $0.74 \pm 0.17$ &$0.86 \pm 0.17$ &$0.89 \pm 0.15$ &$0.85 \pm 0.16$& \control{} < \dashboard{}, \chatxai{}, \chatpersonalized{} \\
	\textbf{Switch Fraction}& 17.65 & \textbf{.001}$^{\dagger\dagger}$& $0.31 \pm 0.34$ &$0.57 \pm 0.41$ &$0.58 \pm 0.43$ &$0.57 \pm 0.41$& \control{} < \dashboard{}, \chatxai{}, \chatpersonalized{}\\
    \rowcolor{gray!15}\textbf{Accuracy-wid}& 2.04 & .563& $0.46 \pm 0.30$ &$0.50 \pm 0.36$ &$0.52 \pm 0.35$ &$0.55 \pm 0.38$& -\\
    \textbf{RAIR}& 10.93 & \textbf{.012}$^{\dagger\dagger}$& $0.35 \pm 0.39$ &$0.50 \pm 0.44$ &$0.60 \pm 0.45$ &$0.52 \pm 0.44$& \control{} < \chatxai{} \\
	\rowcolor{gray!15}\textbf{RSR}& 23.75 & \textbf{.000}$^{\dagger\dagger}$& $0.57 \pm 0.46$ &$0.29 \pm 0.44$ &$0.23 \pm 0.40$ &$0.26 \pm 0.41$&  \control{} > \dashboard{}, \chatxai{}, \chatpersonalized{}\\
    % \textbf{TiA-Trust}& 3.93& .140& $3.00 \pm 0.81$& $3.22 \pm 0.87$& $3.11 \pm 0.85$& -\\
	    \hline
	\end{tabular}
        }
	\end{small}
\end{table*}

% \begin{figure*}[htbp]
%  \centering
%   \subfigure[Accuracy as a measure of the team performance in decision-making.]{\label{fig:estimation-acc}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_accuracy.png}
%  }
%   \subfigure[Accuracy-wid as a measure of the team performance in decision-making.]{\label{fig:estimation-wid}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_accuracy_wid.png}
%  }
%  \subfigure[RAIR as a measure of appropriate reliance.]{\label{fig:estimation-RAIR}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_RAIR.png}
%  }
%   \subfigure[RSR as a measure of appropriate reliance.]{\label{fig:estimation-RSR}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_RSR.png}
%  }
%  \centering
%  \caption{Estimation plots (95\% CI) of user performance and appropriate reliance across the four experimental conditions.
%  }
%  \label{fig-performance-estimation}
%  \Description{Four estimation plots for overall Accuracy, Accuracy-wid, RAIR, and RSR. (a) The estimation plot shows that participants in condition CXAI show slightly better Accuracy in comparison with condition Dashboard and PCXAI. (b) The estimation shows that participants in condition PCXAI show slightly better Accuracy-wid in comparison with condition Dashboard and CXAI. (c) The estimation plot shows that participants in condition CXAI show slightly better RAIR in comparison with condition Dashboard and PCXAI. (d) The estimation shows that participants in condition Dashboard show slightly better RSR in comparison with condition CXAI and PCXAI.}
% \end{figure*}

There is no significant difference in team performance (\ie \textit{Accuracy} and \textit{Accuracy-wid}). 
To interpret our data beyond \textit{p}-values and better understand effect sizes in terms of the overall team performance,
% To interpret how the explainer interface affects team performance, 
we adopted estimation plots~\cite{ho2019moving}  {(shown in supplementary materials, Figure 4)}. Based on the normal distribution sampled for these measures, we can infer the reliance difference based on the mean difference of the estimated distribution.
% , as shown in Figure~\ref{fig-performance-estimation}. 
% Jitter plots show the overall \textit{Accuracy} (Figure~\ref{fig:estimation-acc}) and \textit{Accuracy-wid}  (Figure~\ref{fig:estimation-wid}), and how they distribute, across experimental conditions. 
% Here, we use the no XAI interface as a control group in the plots to make a comparison with all the other experimental conditions. 
We found that: (1) Compared to the \control{} condition, participants %showed a better distribution of accuracy 
in the \chatxai{} condition %, which is reflected by the mean difference distribution. \glcomment{how about: Compared to the \control{} condition, participants in the \chatxai{} condition 
showed a clearly higher mean accuracy.
% , which is reflected by the mean difference in the estimated distribution.}
(2) Participants in the \chatpersonalized{} condition showed slightly better \textit{Accuracy-wid} than the \dashboard{} condition and the \chatxai{} condition.
% ~\glcomment{Another option is to show estimation plots for RAIR and RSR. But I found their distribution is relatively extreme (more 1 and 0 instead of values between)} \ug{Yeah, perhaps add those as additional plots in the repository. Unless the mean difference is still interesting to report via these plots. Can you send those to me on Teams chat and we can decide?}
Similarly, we adopted estimation plots~\cite{ho2019moving} {(cf. supplementary materials, Figure 4)} to draw meaningful interpretations related to our appropriate reliance measures. %~\glcomment{Explain what the “better distribution” in the estimation plots means and move important plots to the main body of the paper (R3).}
% Jitter plots show the overall \textit{RAIR} (Figure~\ref{fig:estimation-RAIR}) and \textit{RSR}  (Figure~\ref{fig:estimation-RSR}), and how they distribute, across experimental conditions. 
% Here, we use the no XAI interface as a control group in the plots to make a comparison with all the other experimental conditions. 
We found that: (1) Compared to the \control{} condition, % participants showed a significantly better distribution of \textit{RAIR} in the \chatxai{} condition, which is reflected by the mean difference distribution. 
%\glcomment{how about: Compared to the \control{} condition, 
participants in the \chatxai{} condition showed a significantly higher  \textit{RAIR}.
% , which is reflected by the mean difference in the estimated distribution.}
At the same time, participants in the \chatxai{} condition showed a slightly higher \textit{RAIR} compared with participants in  \dashboard{} and  \chatpersonalized{} conditions.
(2) Participants in the \dashboard{} and \chatpersonalized{} conditions showed slightly better \textit{RSR} than the \chatxai{} condition.

% \begin{figure*}[htbp]
%  \centering
%   \subfigure[Accuracy as a measure of the team performance in decision-making.]{\label{fig:estimation-acc}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_accuracy.png}
%  }
%   \subfigure[Accuracy-wid as a measure of the team performance in decision-making.]{\label{fig:estimation-wid}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_accuracy_wid.png}
%  }
%  \subfigure[RAIR as a measure of appropriate reliance.]{\label{fig:estimation-RAIR}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_RAIR.png}
%  }
%   \subfigure[RSR as a measure of appropriate reliance.]{\label{fig:estimation-RSR}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_RSR.png}
%  }
%  \centering
%  \caption{Estimation plots (95\% CI) of user performance and appropriate reliance across the four experimental conditions.
%  }
%  \label{fig-performance-estimation}
%  \Description{Two estimation plots for overall Accuracy and Accuracy-wid. (a) The estimation plot shows that participants in condition CXAI show slightly better Accuracy in comparison with condition Dashboard and PCXAI. (b) The estimation shows that participants in condition PCXAI show slightly better Accuracy-wid in comparison with condition Dashboard and CXAI. (c) The estimation plot shows that participants in condition CXAI show slightly better RAIR in comparison with condition Dashboard and PCXAI. (d) The estimation shows that participants in condition Dashboard show slightly better RSR in comparison with condition CXAI and PCXAI.}
% \end{figure*}


% \begin{figure*}[htbp]
%  \centering
%   \subfigure[RAIR as a measure of appropriate reliance.]{\label{fig:estimation-RAIR}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_RAIR.png}
%  }
%   \subfigure[RSR as a measure of appropriate reliance.]{\label{fig:estimation-RSR}
%   \centering
%   \includegraphics[width=0.48\textwidth]{figures/estimation_plot_RSR.png}
%  }
%  \centering
%  \caption{Estimation plots (95\% CI) of appropriate reliance across the four experimental conditions.
%  }
%  \label{fig-appropriate-reliance-estimation}
%  \Description{Two estimation plots for overall RAIR and RSR. (a) The estimation plot shows that participants in condition CXAI show slightly better RAIR in comparison with condition Dashboard and PCXAI. (b) The estimation shows that participants in condition Dashboard show slightly better RSR in comparison with condition CXAI and PCXAI.}
% \end{figure*}

% Similarly, we adopted estimation plots~\cite{ho2019moving} for appropriate reliance measures. 
% % Jitter plots show the overall \textit{RAIR} (Figure~\ref{fig:estimation-RAIR}) and \textit{RSR}  (Figure~\ref{fig:estimation-RSR}), and how they distribute, across experimental conditions. 
% % Here, we use the no XAI interface as a control group in the plots to make a comparison with all the other experimental conditions. 
% We found that: (1) Compared to the \control{} condition, participants showed a significantly better distribution of \textit{RAIR} in the \chatxai{} condition, which is reflected by the mean difference distribution. 
% At the same time, participants in the condition \chatxai{} showed a slightly better distribution of \textit{RAIR} compared with participants in condition \dashboard{} and condition \chatpersonalized{}.
% (2) Participants in the \dashboard{} and \chatpersonalized{} condition showed slightly better \textit{RSR} than the the \chatxai{} condition.

\subsubsection{\textbf{H4}: effect of {evaluative conversation} on user trust and appropriate reliance}

% H4: Personalizing explanations and adaptive steering of conversations in the conversational XAI interface will increase user trust and appropriate reliance on an AI system.
According to results reported in Section~\ref{sec-h2} and Section~\ref{sec-h3}, 
% shown in Table~\ref{tab:H2} and Table~\ref{tab:res-reliance}, 
no significant difference in user trust and appropriate reliance was found between experimental condition \chatxai{} and \chatpersonalized{}. Thus, \textbf{H4} is not supported. 
% \glcomment{save space}

% \ug{Before the final submission ensure that tables and figures are positioned close to where they are referred. At the moment, this may have been disrupted due to the comments.}


\subsection{\revise{Follow-up Study Using an LLM Agent: Beyond Rule-based Conversational XAI }}
\label{sec-llm-agent}

%\reviewer{R3 comment: I appreciate the added LLM agent condition. But why it is a representative condition of personalization? Why it offer more personalization than the previous two conditions? The logic blurs here.}

% In the main study, we found that the conversational user interfaces did not significantly impact user trust or appropriate reliance on the AI system. 
{In the main study, we found that conversational user interfaces did not lead to a significant difference in user understanding, user trust, or appropriate reliance compared to the XAI dashboard.}
%does not work as expected. 
One potential cause can be that the conversational user interfaces of condition \chatxai{} and \chatpersonalized{} are based on rule-based agents, which only provide pre-defined responses based on templates. 
Such a design ensures progress in conversational interaction but lacks the flexibility to deal with user needs in a bilateral human-like conversation. %, which may bring users unnatural experiences and less knowledge to learn after several trials. 
% Once the participants realized that our conversational user interface could only provide robot-like responses, user trust and reliance on the AI system may be impacted. 
To address such concerns and further our understanding of the impact of {flexible interaction and enhanced conversation quality in the conversational XAI interface}%\glcomment{We previously use ``on user reliance'', but it seems our results include all dimensions we used in our study. Is `flexible interaction' clear, I mean users can be more flexible in expressing their information needs. This part I feel a bit tricky to describe within several words.}
% personalization
% ~\glcomment{conversational decision support? To discuss, whether we can highlight the evaluative perspectives here?} 
%and adaptive steering \glcomment{discuss: shall we remove ``adaptive steering'' here?}
% on user reliance
, we built another conversational XAI interface powered by large language model agents. 
The benefits of introducing large language model agents are two-fold: (1) LLMs have shown promising user query understanding capability, which enables understanding user information needs and generating coherent and high-quality personalized conversation responses~\cite{zhao2023survey}. (2) When equipped with XAI methods as potential tools, LLM agents can provide suitable XAI responses on demand, which may provide a better user experience {(\eg more flexible expression of information needs and high-quality text responses based on XAI outcomes)}.
% \glcomment{add citations}}
% \glcomment{Further motivate the follow-up study to understand the impact of personalization}

The entire procedure of condition \ie \chatagent{} is identical to condition \chatxai{} and \chatpersonalized{} barring one difference. 
The conversational XAI interface in this case is powered by an LLM agent instead of a rule-based agent. 
Our implementation of the LLM agent is based on autogen~\cite{wu2023autogen} and GPT-4. 
Given user queries, the LLM agent-based conversational XAI  transforms user intents into pre-defined explainers and elaborates on the generated explanations to generate coherent text responses. 
We also provide the five hint questions (as shown in Table~\ref{tab:xai_conversation}) to trigger potential XAI responses during the conversation in a randomized order on every task. %Besides this, 
Users can ask the LLM agent any questions using the textual input. On average, each task consumes 13 API calls to obtain GPT-4 responses, including generating reply messages and XAI usage. %\glcomment{shall we mention how much we spend in total for this? seems not very important detail}
For more implementation details of our LLM agent-based conversational XAI interface, readers can refer to our supplementary materials. 
For ease of comparison with other conditions in an exploratory fashion, we recruited 61 valid participants from Prolific (with compensation and filter criteria identical to our main study). 
%\glcomment{In the appendix, we can show some conversation records to tell the difference across conditions.} \ug{Good idea!}

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/reliance_plot.pdf}
    \caption{Bar plot showing the behavior-based variables across all conditions. Only significant results (\ie post-hoc Mann–Whitney test) related to condition \chatagent{} are highlighted. (*: $p < 0.0125$; **: $p < 0.001$). The error bars represent the $95\%$ confidence interval.} 
    \label{fig:reliance_llm_agent}
    \Description{Bar plots for behavior-based variables (accuracy, accuracy-wid, agreement faction, switch fraction, RAIR, and RSR) across all conditions. The significant results associated with the condition LLM Agent are annotated.}
\end{figure*}

Following the hypothesis testing used in Section~\ref{sec-hyp-test}, we compared user understanding, user trust, and user (appropriate) reliance against the previous conditions. 
We find that: (1) In user understanding,  \chatagent{} condition showed significantly worse \textit{objective user understanding} than the \dashboard{}, \chatxai{}, and \chatpersonalized{} conditions. 
Besides this, there is no significant difference across conditions with other measures of user understanding. 
(2) In user trust, we found that participants in the \chatagent{} condition showed a consistent but non-significant trend across all measures: \control{} < \chatagent{} < \dashboard{}, \chatxai{}, \chatpersonalized{}. 
% Combined with the finding that participants in condition \dashboard{}, \chatxai{} and \chatpersonalized{} showed significantly higher TiA-U/P than condition \control{}. 
(3) As for user reliance (cf. Figure~\ref{fig:reliance_llm_agent}), participants in the \chatagent{} condition showed significantly higher \textit{Agreement Fraction} and \textit{Switch Fraction} than in the \control{} condition. %which keeps our main finding in hypothesis testing of \textbf{H3}. 
However, we found that participants in the \chatagent{} condition showed significantly worse RSR compared to the \control{} and \dashboard{} conditions, which indicates that the \chatagent{} condition led to %from more
severe over-reliance on the AI advice.
% \glcomment{To highlight the results for appropriate reliance, I guess it would be better to visualize with a table or figure here}
% \paratitle{Conversation Analysis}


% \paratitle{trust, reliance, and user understanding} \glcomment{Shall we add the results into previous hypothesis test? I have new hypothesis test results}

% \begin{table*}[hbpt]
% % the environment \color{blue} change all cell color
% 	\centering
% 	\caption{Summary of significant results in all hypothesis testing.\glcomment{Now it looks a bit weird. Is it problematic to gather hypothesis test and follow-up test together? Think about more attractive way (figure or table)}}
% 	\label{tab:res-summary}%
% 	\begin{small}
%     \scalebox{0.95}{
% 	\begin{tabular}{c | c | c | c}
% 	    \hline
% 	    \textbf{Hypothesis}& \textbf{Category}& \textbf{Dependent Variables}& Post-hoc results\\
%      % \cline{4-7}
%      % &  & & \control& \dashboard{}& \chatxai{}& \chatpersonalized{}& \\
% 	    \hline \hline
%     \textbf{H1}& \textbf{Understanding}& \rowcolor{gray!15}\textbf{objective feature understanding} & \dashboard{}, \chatxai{}, \chatpersonalized{} > \chatagent{}\\	
%     % \cline{3-4}
%     \hline
%     \textbf{H2}& \textbf{Trust}& \textbf{TiA-U/P} & \control{} < \dashboard{}, \chatxai{}, \chatpersonalized{}\\	
%     % \cline{2-4}
%     \hline
%  \multirow{5}{*}{\textbf{H3}}& \multirow{5}{*}{\textbf{Reliance}} & \rowcolor{gray!15}\textbf{Agreement Fraction}& \control{} < \dashboard{}, \chatxai{}, \chatpersonalized{} \\
%  % \cline{3-4}
% 	& &\textbf{Switch Fraction}& \control{} < \dashboard{}, \chatxai{}, \chatpersonalized{}\\
%  % \cline{3-4}
%     & &\rowcolor{gray!15}\textbf{RAIR}& \control{} < \chatxai{} \\ 
% 	& &\multirow{2}{*}{\textbf{RSR}}&  \control{} > \dashboard{}, \chatxai{}, \chatpersonalized{}, \chatagent{}\\
% 	& & &  \dashboard{} > \chatagent{}\\
% 	    \hline
% 	\end{tabular}
%  }
% 	\end{small}
% \end{table*}


\subsection{Exploratory Analyses}
For more exploratory analyses of covariates, readers can refer to our supplementary materials. 
% ~\glcomment{Provide more analysis of qualitative data, including users’ usage patterns and user behavior (R2, R3).}

% \begin{table}[htbp]
% 	\centering
% 	\caption{Correlation of covariates and dependent variables. ``$\dagger$'' and ``$\dagger\dagger$'' indicate the effect of the variable is significant at the level of 0.05 and 0.0125, respectively.
%  % ~\glcomment{we may consider add one column for DV category: User Understanding, Trust, Reliance. We can consider deleting the columns for ML background, as no significant correlation is found.}
%  }
% 	\label{tab:correlation}%
% 	\begin{small}
% 	\begin{tabular}{r | c c | c c| c c | c c }
% 	    \hline
% 	    \textbf{Covariates}&	\multicolumn{2}{c|}{\textbf{Propensity to Trust}}& \multicolumn{2}{c|}{\textbf{TiA-Familiarity}} & \multicolumn{2}{c|}{\textbf{ATI}} & \multicolumn{2}{c}{\textbf{ML background}}\\
% 	    \hline
% 	    \textbf{Dependent Variables}& $r$& $p$& $r$& $p$& $r$& $p$& $r$& $p$ \\
% 	    \hline \hline
%             Perceived Feature Understanding & 0.305 & \textbf{.000}$^{\dagger\dagger}$& 0.061 & .408& 0.134 & .070& -0.012 & .872\\
%             Explanation Completeness & 0.322 & \textbf{.000}$^{\dagger\dagger}$& 0.010 & .895& 0.007 & .925& 0.088 & .234\\
%             Explanation Coherence & 0.323 & \textbf{.000}$^{\dagger\dagger}$& 0.147 & .047$^{\dagger}$& 0.116 & .118& 0.091 & .220\\
%             Explanation Clarity & 0.409 & \textbf{.000}$^{\dagger\dagger}$& 0.028 & .709& 0.121 & .101& 0.089 & .228\\
%             Learning Effect Across Tasks & 0.175 & .017$^{\dagger}$& 0.136 & .066& 0.130 & .078& 0.129 & .082\\
%             Understanding of System & 0.318 & \textbf{.000}$^{\dagger\dagger}$& 0.068 & .357& 0.201 & \textbf{.006}$^{\dagger\dagger}$& 0.025 & .738\\
%             Explanation Usefulness & 0.375 & \textbf{.000}$^{\dagger\dagger}$& 0.096 & .194& 0.147 & .047$^{\dagger}$& 0.036 & .623\\
%             Objective Feature Understanding & 0.177 & .016$^{\dagger}$& -0.114 & .123& 0.027 & .716& 0.045 & .544\\
%             \hline
%             TiA-R/C & 0.637 & \textbf{.000}$^{\dagger\dagger}$& 0.089 & .166& 0.151 & .018$^{\dagger}$& 0.095 & .137\\
%             TiA-U/P & 0.426 & \textbf{.000}$^{\dagger\dagger}$& 0.057 & .376& 0.284 & \textbf{.000}$^{\dagger\dagger}$& 0.147 & .021$^{\dagger}$\\
%             TiA-Trust & 0.764 & \textbf{.000}$^{\dagger\dagger}$& 0.201 & \textbf{.002}$^{\dagger\dagger}$& 0.124 & .052& 0.096 & .134\\
%             \hline
%             Accuracy & 0.121 & .058& 0.094 & .142& -0.030 & .637& -0.001 & .990\\
%             Agreement Fraction & 0.272 & \textbf{.000}$^{\dagger\dagger}$& 0.037 & .563& 0.036 & .576& -0.007 & .917\\
%             Switch Fraction & 0.172 & \textbf{.007}$^{\dagger\dagger}$& -0.034 & .601& -0.007 & .909& 0.086 & .179\\
%             Accuracy-wid & 0.058 & .366& 0.079 & .217& -0.067 & .295& 0.086 & .181\\
%             RAIR & 0.126 & .049$^{\dagger}$& 0.014 & .828& -0.044 & .489& 0.068 & .289\\
%             RSR & -0.224 & \textbf{.000}$^{\dagger\dagger}$& -0.003 & .968& -0.069 & .283& -0.065 & .312\\
% 	    \hline
% 	\end{tabular}%
% 	\end{small}
% \end{table}%

% \subsubsection{Impact of Covariates}
% As shown in the analysis for \textbf{H2} (cf. Table~\ref{tab:H2}), covariates like TiA-Propensity to Trust and ATI have shown some impact on user trust. 
% To further analyze the impact of covariates on human-AI decision making, we conducted Spearman rank-order tests between covariates and all categories of dependent variables. The results are shown in Table~\ref{tab:correlation}. 
% We have the following main findings: (1) Overall, \textit{TiA-Propensity to Trust} significantly positively impacted most dependent variables in user understanding, trust, and reliance categories. 
% (2) While the propensity to trust positively correlated with user reliance (\ie \textit{Agreement Fraction} and \textit{Switch Fraction}), it negatively affects \textit{RSR}. In other words, some participants with a higher propensity to trust tend to over-rely on the AI system. 
% (3) \textit{TiA-Familiarity} and \textit{ATI} only showed some positive impact on user understanding and user trust. No significant correlation was found for user reliance. 
% (4) We did not find a significant correlation for the covariate of \textit{ML background}.

% \begin{table}[htbp]
% 	\centering
% 	\caption{Correlation of covariates and dependent variables. ``$\dagger$'' and ``$\dagger\dagger$'' indicate the effect of the variable is significant at the level of 0.05 and 0.0125, respectively.
%  % ~\glcomment{we may consider add one column for DV category: User Understanding, Trust, Reliance. We can consider deleting the columns for ML background, as no significant correlation is found.}
%  }
% 	\label{tab:correlation}%
% 	\begin{small}
% 	\begin{tabular}{r | c c | c c| c c | c c }
% 	    \hline
% 	    \textbf{Covariates}&	\multicolumn{2}{c|}{\textbf{Propensity to Trust}}& \multicolumn{2}{c|}{\textbf{TiA-Familiarity}} & \multicolumn{2}{c|}{\textbf{ATI}} & \multicolumn{2}{c}{\textbf{ML background}}\\
% 	    \hline
% 	    \textbf{Dependent Variables}& $r$& $p$& $r$& $p$& $r$& $p$& $r$& $p$ \\
% 	    \hline \hline
%             Perceived Feature Understanding & 0.305 & \textbf{.000}$^{\dagger\dagger}$& 0.061 & .408& 0.134 & .070& -0.012 & .872\\
%             Explanation Completeness & 0.322 & \textbf{.000}$^{\dagger\dagger}$& 0.010 & .895& 0.007 & .925& 0.088 & .234\\
%             Explanation Coherence & 0.323 & \textbf{.000}$^{\dagger\dagger}$& 0.147 & .047$^{\dagger}$& 0.116 & .118& 0.091 & .220\\
%             Explanation Clarity & 0.409 & \textbf{.000}$^{\dagger\dagger}$& 0.028 & .709& 0.121 & .101& 0.089 & .228\\
%             Learning Effect Across Tasks & 0.175 & .017$^{\dagger}$& 0.136 & .066& 0.130 & .078& 0.129 & .082\\
%             Understanding of System & 0.318 & \textbf{.000}$^{\dagger\dagger}$& 0.068 & .357& 0.201 & \textbf{.006}$^{\dagger\dagger}$& 0.025 & .738\\
%             Explanation Usefulness & 0.375 & \textbf{.000}$^{\dagger\dagger}$& 0.096 & .194& 0.147 & .047$^{\dagger}$& 0.036 & .623\\
%             Objective Feature Understanding & 0.177 & .016$^{\dagger}$& -0.114 & .123& 0.027 & .716& 0.045 & .544\\
%             \hline
%             TiA-R/C & 0.637 & \textbf{.000}$^{\dagger\dagger}$& 0.089 & .166& 0.151 & .018$^{\dagger}$& 0.095 & .137\\
%             TiA-U/P & 0.426 & \textbf{.000}$^{\dagger\dagger}$& 0.057 & .376& 0.284 & \textbf{.000}$^{\dagger\dagger}$& 0.147 & .021$^{\dagger}$\\
%             TiA-Trust & 0.764 & \textbf{.000}$^{\dagger\dagger}$& 0.201 & \textbf{.002}$^{\dagger\dagger}$& 0.124 & .052& 0.096 & .134\\
%             \hline
%             Accuracy & 0.121 & .058& 0.094 & .142& -0.030 & .637& -0.001 & .990\\
%             Agreement Fraction & 0.272 & \textbf{.000}$^{\dagger\dagger}$& 0.037 & .563& 0.036 & .576& -0.007 & .917\\
%             Switch Fraction & 0.172 & \textbf{.007}$^{\dagger\dagger}$& -0.034 & .601& -0.007 & .909& 0.086 & .179\\
%             Accuracy-wid & 0.058 & .366& 0.079 & .217& -0.067 & .295& 0.086 & .181\\
%             RAIR & 0.126 & .049$^{\dagger}$& 0.014 & .828& -0.044 & .489& 0.068 & .289\\
%             RSR & -0.224 & \textbf{.000}$^{\dagger\dagger}$& -0.003 & .968& -0.069 & .283& -0.065 & .312\\
% 	    \hline
% 	\end{tabular}%
% 	\end{small}
% \end{table}%

% \subsubsection{The Impact of User Understanding, \gladd{Explanation Utility,} and User Trust on User \gladd{Performance and} Reliance}
% \glcomment{How about `Correlation analysis between perception-based variables and behavior-based variables'? I think current title is too long and complex}
\subsubsection{{The Impact of User Perceptions on Their Behavior}} Prior work has shown that user trust can substantially affect user reliance behaviors~\cite{lee2004trust,Tolmeijer-UMAP-2021}. 
% In this work, we expect that a conversational user interface can help improve user understanding of the AI system and further promote user trust and appropriate reliance. 
To further analyze how {perception-based variables (\ie user trust, user understanding, and explanation utility)} affect team performance and user reliance behaviors {(\ie behavior-based variables)}, we conducted Spearman rank-order tests between {corresponding categories of variables}.
% the dependent variables of the user understanding and user trust categories with the dependent variables pertaining to the categories of performance, reliance, and appropriate reliance. \glcomment{This description seems a bit complex, shall we simply mention ``Spearman rank-order tests between corresponding categories of variables''}
%~\glcomment{To check, whether this sent is problematic}
The results are presented in Table~\ref{tab:exploratory_reliance_correlation}. 

% \begin{table}[htbp]
% 	\centering
% 	\caption{Correlation of covariates and dependent variables. ``$\dagger$'' and ``$\dagger\dagger$'' indicate the effect of variable is significant at the level of 0.05 and 0.0125, respectively.
%  }
% 	\label{tab:exploratory_reliance_correlation}%
% 	\begin{footnotesize}
%     \scalebox{0.92}{
% 	\begin{tabular}{r | c c | c c| c c | c c | c c | c c}
% 	    \hline
% 	    \textbf{Performance / Reliance}&	\multicolumn{2}{c|}{\textbf{Accuracy}}& \multicolumn{2}{c|}{\textbf{Accuracy-wid}} & \multicolumn{2}{c|}{\textbf{Agreement Fraction}} & \multicolumn{2}{c|}{\textbf{Switch Fraction}}& \multicolumn{2}{c|}{\textbf{RAIR}} & \multicolumn{2}{c}{\textbf{RSR}}\\
% 	    \hline
% 	    \textbf{Understanding / Trust}& $r$& $p$& $r$& $p$& $r$& $p$& $r$& $p$& $r$& $p$& $r$& $p$ \\
% 	    \hline \hline
%             Perceived Feature Understanding & 0.118 & .110& 0.050 & .504& 0.331 & \textbf{.000}$^{\dagger\dagger}$& 0.195 & \textbf{.008}$^{\dagger\dagger}$& 0.172 & .020$^{\dagger}$& -0.333 & \textbf{.000}$^{\dagger\dagger}$\\
%             Explanation Completeness & 0.144 & .052& 0.160 & .030$^{\dagger}$& 0.207 & \textbf{.005}$^{\dagger\dagger}$& 0.217 & \textbf{.003}$^{\dagger\dagger}$& 0.244 & \textbf{.001}$^{\dagger\dagger}$& -0.181 & .014$^{\dagger}$\\
%             Explanation Coherence & 0.159 & .031$^{\dagger}$& 0.000 & .996& 0.361 & \textbf{.000}$^{\dagger\dagger}$& 0.080 & .281& 0.019 & .793& -0.281 & \textbf{.000}$^{\dagger\dagger}$\\
%             Explanation Clarity & 0.052 & .481& -0.084 & .257& 0.276 & \textbf{.000}$^{\dagger\dagger}$& 0.108 & .145& 0.071 & .340& -0.293 & \textbf{.000}$^{\dagger\dagger}$\\
%             Learning Effect Across Tasks & 0.052 & .481& -0.056 & .452& 0.190 & \textbf{.010}$^{\dagger\dagger}$& 0.039 & .600& 0.044 & .557& -0.193 & \textbf{.009}$^{\dagger\dagger}$\\
%             Understanding of System & 0.159 & .031$^{\dagger}$& -0.071 & .341& 0.217 & \textbf{.003}$^{\dagger\dagger}$& 0.002 & .973& -0.038 & .609& -0.213 & \textbf{.004}$^{\dagger\dagger}$\\
%             Explanation Usefulness & 0.160 & .030$^{\dagger}$& 0.059 & .425& 0.443 & \textbf{.000}$^{\dagger\dagger}$& 0.261 & \textbf{.000}$^{\dagger\dagger}$& 0.199 & \textbf{.007}$^{\dagger\dagger}$& -0.383 & \textbf{.000}$^{\dagger\dagger}$\\
%             Objective Feature Understanding & 0.320 & \textbf{.000}$^{\dagger\dagger}$& 0.225 & \textbf{.002}$^{\dagger\dagger}$& 0.500 & \textbf{.000}$^{\dagger\dagger}$& 0.410 & \textbf{.000}$^{\dagger\dagger}$& 0.321 & \textbf{.000}$^{\dagger\dagger}$& -0.380 & \textbf{.000}$^{\dagger\dagger}$\\
%             \hline
%             TiA-R/C & 0.197 & \textbf{.007}$^{\dagger\dagger}$& 0.105 & .156& 0.305 & \textbf{.000}$^{\dagger\dagger}$& 0.224 & \textbf{.002}$^{\dagger\dagger}$& 0.174 & .018$^{\dagger}$& -0.273 & \textbf{.000}$^{\dagger\dagger}$\\
%             TiA-U/P & 0.157 & .033$^{\dagger}$& 0.007 & .920& 0.319 & \textbf{.000}$^{\dagger\dagger}$& 0.142 & .054& 0.085 & .250& -0.272 & \textbf{.000}$^{\dagger\dagger}$\\
%             TiA-Trust & 0.199 & \textbf{.007}$^{\dagger\dagger}$& 0.057 & .439& 0.332 & \textbf{.000}$^{\dagger\dagger}$& 0.221 & \textbf{.003}$^{\dagger\dagger}$& 0.185 & \textbf{.012}$^{\dagger\dagger}$& -0.282 & \textbf{.000}$^{\dagger\dagger}$\\
% 	    \hline
% 	\end{tabular}%
%  }
% 	\end{footnotesize}
% \end{table}%

\begin{table*}[htbp]
	\centering
	\caption{Correlation between {perception-based variables (\ie user understanding, explanation utility, and user trust) and behavior-based variables}. ``$\dagger$'' and ``$\dagger\dagger$'' indicate the effect of the variable is significant at the level of 0.05 and 0.0125, respectively.%\glcomment{The only concern for RSR. Shall we calculate it only when the user shows valid patterns? Now we use all users}}
 }
	\label{tab:exploratory_reliance_correlation}%
	\begin{small}
    % \scalebox{0.9}{
    % \revise{
	\begin{tabular}{r | c c | c c| c c | c c | c c | c c}
	    \hline
	    \textbf{Behavior-based Variables}&	\multicolumn{2}{c|}{\textbf{Accuracy}}& \multicolumn{2}{c|}{\textbf{Accuracy-wid}} & \multicolumn{2}{c|}{\textbf{Agreement Fraction}} & \multicolumn{2}{c|}{\textbf{Switch Fraction}}& \multicolumn{2}{c|}{\textbf{RAIR}} & \multicolumn{2}{c}{\textbf{RSR}}\\
	    \hline
	    \textbf{Perception-based Variables}& $r$& $p$& $r$& $p$& $r$& $p$& $r$& $p$& $r$& $p$& $r$& $p$ \\
	    \hline \hline
            Perceived Feature Understanding& 0.045 & .484& -0.024 & .709& 0.254 &\textbf{.000}$^{\dagger\dagger}$& 0.117 & .067& 0.096 & .135& -0.293 &\textbf{.000}$^{\dagger\dagger}$\\
            Objective Feature Understanding & 0.332 &\textbf{.000}$^{\dagger\dagger}$& 0.195 &\textbf{.002}$^{\dagger\dagger}$& 0.469 &\textbf{.000}$^{\dagger\dagger}$& 0.322 &\textbf{.000}$^{\dagger\dagger}$& 0.269 &\textbf{.000}$^{\dagger\dagger}$& -0.297 &\textbf{.000}$^{\dagger\dagger}$\\
            Learning Effect Across Tasks & 0.084 & .192& -0.085 & .184& 0.170 &\textbf{.008}$^{\dagger\dagger}$& -0.006 & .931& 0.007 & .913& -0.135 & .035$^{\dagger}$\\
            Understanding of System & 0.114 & .076& -0.083 & .197& 0.157 & .014$^{\dagger}$& 0.010 & .877& -0.017 & .795& -0.153 & .016$^{\dagger}$\\
            \hline
            Explanation Completeness & 0.050 & .435& 0.056 & .387& 0.146 & .022$^{\dagger}$& 0.142 & .026$^{\dagger}$& 0.157 & .014$^{\dagger}$& -0.170 &\textbf{.007}$^{\dagger\dagger}$\\
            Explanation Coherence& 0.107 & .095& -0.030 & .643& 0.270 &\textbf{.000}$^{\dagger\dagger}$& 0.068 & .286& 0.005 & .935& -0.218 &\textbf{.001}$^{\dagger\dagger}$\\
            Explanation Clarity & 0.002 & .973& -0.111 & .083& 0.190 &\textbf{.003}$^{\dagger\dagger}$& 0.081 & .204& 0.042 & .514& -0.235 &\textbf{.000}$^{\dagger\dagger}$\\
            Explanation Usefulness & 0.125 & .051& 0.081 & .206& 0.361 &\textbf{.000}$^{\dagger\dagger}$& 0.266 &\textbf{.000}$^{\dagger\dagger}$& 0.229 &\textbf{.000}$^{\dagger\dagger}$& -0.300 &\textbf{.000}$^{\dagger\dagger}$\\
            % Objective Feature Understanding & 0.332 &\textbf{.000}$^{\dagger\dagger}$& 0.195 &\textbf{.002}$^{\dagger\dagger}$& 0.469 &\textbf{.000}$^{\dagger\dagger}$& 0.322 &\textbf{.000}$^{\dagger\dagger}$& 0.269 &\textbf{.000}$^{\dagger\dagger}$& -0.297 &\textbf{.000}$^{\dagger\dagger}$\\
            \hline
            TiA-R/C& 0.127 & .047$^{\dagger}$& 0.090 & .162& 0.224 &\textbf{.000}$^{\dagger\dagger}$& 0.195 &\textbf{.002}$^{\dagger\dagger}$& 0.175 &\textbf{.006}$^{\dagger\dagger}$& -0.200 &\textbf{.002}$^{\dagger\dagger}$\\
            TiA-U/P & 0.099 & .123& 0.051 & .430& 0.210 &\textbf{.001}$^{\dagger\dagger}$& 0.132 & .038$^{\dagger}$& 0.125 & .051& -0.182 &\textbf{.004}$^{\dagger\dagger}$\\
            TiA-Trust & 0.145 & .024$^{\dagger}$& 0.032 & .617& 0.254 &\textbf{.000}$^{\dagger\dagger}$& 0.164 &\textbf{.010}$^{\dagger\dagger}$& 0.152 & .017$^{\dagger}$& -0.203 &\textbf{.001}$^{\dagger\dagger}$\\
	    \hline
	\end{tabular}%
 % }
	\end{small}
\end{table*}%

We found that: (1) \textit{Agreement Fraction} and \textit{RSR} are significantly correlated with most dimensions of user understanding, explanation utility, and user trust. However, these dimensions are positively correlated with \textit{Agreement Fraction} but negatively correlated with \textit{RSR}. 
{This suggests that the improved user understanding, {explanation utility,} and user trust with XAI interfaces can partially explain the increased over-reliance on the AI system.} 
% \gladd{(2) The perceived usefulness of explanations will contribute to higher user reliance and RAIR, meanwhile it negatively impact RSR. }
(2) While user trust dimension \textit{TiA-R/C} and \textit{TiA-Trust} positively correlated with reliance measures (\textit{Agreement Fraction} and \textit{Switch Fraction}), and \textit{RAIR}, they negatively correlated with \textit{RSR}. As a result, they do not show a significant correlation with \textit{Accuracy-wid}. 
{This corroborates that higher user trust in the AI system does not necessarily translate into appropriate reliance behaviors.}
%\glcomment{The sents in orange color are kind of discussion. If you think it would be better to show them in discussion, we can comment them out.}
(3) Overall, \textit{Objective Feature Understanding} seems useful to facilitate appropriate reliance. 
With a higher \textit{objective Feature Understanding}, participants demonstrate better team performance and higher reliance. 
Although it still contributes to over-reliance (reflected by negative correlation with \textit{RSR}), it shows a more positive impact on appropriate reliance (\ie \textit{Accuracy-wid} and \textit{RAIR}). {In comparison, the positive impact of \textit{Explanation Usefulness}, \textit{TiA-R/C}, and \textit{TiA-Trust} on mitigating under-reliance (\ie positive correlation with \textit{RAIR}) get canceled by the side effect of over-reliance (\ie negative correlation with \textit{RSR}). As a result, these variables do not significantly contribute to team performance.}
%\glcomment{I update the measures with new conditions. The conclusions are nearly the same}

% While we observed users in condition \chatxai{} and \chatpersonalized{} showed slightly better user understanding and user trust, there is no clear improvement on appropriate reliance

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/confidence_dynamics.pdf}
    \caption{Line plot illustrating the confidence dynamics among users after receiving the AI advice (and explanations). The orange line and blue line illustrate the confidence dynamics before and after receiving AI advice (and explanations), respectively.}
    \label{fig:confidence_dynamics}
    \Description{Four subfigures illustrate the initial user confidence and final user confidence across four experimental conditions. Overall, we found that participants reported a higher confidence after they had access to AI advice. A distinct trend was observed in the \chatxai{} condition, where the reported confidence appears to converge after five tasks. }
\end{figure*}

\subsubsection{Confidence Dynamics}
% \glcomment{We can compare user confidence across conditions to check whether users with conversational user interface showed higher confidence.}
%\glcomment{Discuss why PCXAI cannot provide different confidence dynamics (R3). - we may frame it with the new condition;}
As shown in Figure~\ref{fig:confidence_dynamics}, we illustrate the confidence dynamics of participants in each condition along with the task order. 
In general, we found that participants reported a higher confidence after being exposed to AI advice and explanations. 
While participants in the \control{} condition, the \dashboard{} condition, and the \chatpersonalized{} condition reported a fluctuating trend of confidence along the task order, participants in the \chatxai{} condition reported a relatively clear ascending trend of confidence both before and after the AI advice (and explanations). 
Participants in the \chatagent{} condition showed a clear upward and then downward trend in their confidence related to their final decisions. %It seems that these 
This suggests that participants in this condition first developed over-confidence in the AI system and then calibrated their confidence.  
Interestingly, we observed that the confidence dynamics of participants in the \chatxai{} condition converge after a few tasks. 
The narrow confidence gap before and after receiving AI advice may indicate that participants in the \chatxai{} condition {calibrate their confidence in the AI advice, which reflects a better understanding of the AI system}.
% have developed a better 
% % more comprehensive\ug{better?} 
% understanding of the AI system. \glcomment{I find it not very straightforward to argue a better understanding. But shall we claim more calibrated confidence? which can reflect a better understanding.}
%and can roughly guess the AI prediction.
%From this standpoint, our findings suggest that the conversational XAI interface did help participants better understand the AI system. \glcomment{Are previous arguments still reasonable? I found the LLM Agent condition also shows a large gap between initial and final confidence on most tasks. And they also achieve the worst object user understanding among all conditions with XAI.}
%~\glcomment{Are the previous three sentences clear? Shall we rephrase it? To do more comparison of confidence between conditions?}
To compare the confidence across conditions, we conducted ANOVA tests for both initial confidence (average across tasks) and final confidence (average across tasks). 
Although the \chatxai{}, \chatpersonalized{}, and \chatagent{} conditions showed slightly better user confidence on average, we found no significant differences across conditions. %\ug{This is nice!}
%\glcomment{I tried Earth Mover's Distance (EMD) / Wasserstein Distance to assess the distribution distance between confidence vectors (before and after XAI); there are no significant differences across conditions.} \ug{Got it, thanks for checking!}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.48]{figures/confidence.pdf}
%     \caption{Line plot illustrating the confidence dynamics among users after receiving the AI advice (and explanations). The orange line and blue line illustrate the confidence dynamics before and after receiving AI advice (and explanations), respectively.}
%     \label{fig:confidence_dynamics}
%     \Description{Four subfigures illustrate the initial user confidence and final user confidence across four experimental conditions. Overall, we found that participants reported a higher confidence after they had access to AI advice. A distinct trend was observed in the \chatxai{} condition, where the reported confidence appears to converge after five tasks. }
% \end{figure}

% \subsubsection{Usage of Different XAI methods}
% For participants in the condition \chatxai{} and \chatpersonalized{}, we analyzed their chat journey to understand users information needs by usage of XAI methods. 
% In our analysis, the popularity order of the five explainers are: global explanation (\ie PDP, $46.5\%$ of total usage), SHAP ($24.4\%$ of total usage), WhatIf ($13.0\%$ of total usage), DecisionTree ($10.0\%$ of total usage), Counterfactual (\ie MACE, $6.1\%$ of total usage).
% ~\glcomment{Currently, the statistics come from the metadata. There are some problems if we want to analyze the order of explainers. For example, I never found Decision Tree explainer in the chat journey. If this part is very limited, we can show it in the descriptive statistics}

% \paratitle{General User Habits for XAI usage}. \glcomment{Dynamic Path graph? Maybe only the first two to three steps. Wait for Nilay responses}

\subsubsection{Further Analysis of User Engagement} 
%One important assumption of the superiority of the conversational XAI interface over the XAI dashboard is higher user engagement. 
%To verify this, 
We measured subjective user engagement reported by each participant in our study using the UES-SF questionnaire~\cite{o2018practical}. The distribution of user engagement across the different experimental conditions was as follows: \control{} ($M = 3.15, SD = 0.72$), \dashboard{} ($M = 3.33, SD = 0.66$), \chatxai{} ($M = 3.20, SD = 0.63$), \chatpersonalized{} ($M = 3.28, SD = 0.67$), \chatagent{} ($M = 3.44, SD = 0.71$). 
% An ANCOVA analysis revealed no significant difference in user engagement across the different conditions. 
While participants in the \chatagent{} condition reported slightly higher engagement with the XAI interface, we found this to be non-significant (based on ANOVA analysis).

% \begin{table}[htbp]
% 	\centering
% 	\caption{Kruskal-Wallis H-test results for XAI usages on \chatxai{} and \chatpersonalized{}. }
% 	\label{tab:personalization}%
%         % \scalebox{0.95}{
% 	\begin{tabular}{c | c c | c  c }
% 	    \hline
%             \textbf{XAI Method}& $H$& $p$& $M \pm SD$ (\chatxai{})& $M \pm SD$ (\chatpersonalized{})\\
%             \hline
%             \hline
%             \textbf{PDP}& 0.09& .769& 13.5 $\pm$ 7.3& \textbf{14.1 $\pm$ 8.5} \\
%             \textbf{SHAP}& 3.12& .077& 6.7 $\pm$ 3.7& \textbf{7.8 $\pm$ 3.3}\\
%             \textbf{MACE}& 0.06& .801& 1.8 $\pm$ 1.9& 1.8 $\pm$ 1.9\\
%             \textbf{Decision Tree}& 0.06& .801& 2.8 $\pm$ 3.0& \textbf{3.1 $\pm$ 3.3}\\
%             \textbf{What-If}& 0.26& .613& \textbf{4.1 $\pm$ 4.2}& 3.6 $\pm$ 3.4\\
% 	    \hline
% 	\end{tabular}
%     % }%
% \end{table}%

\subsubsection{Further Analysis of {Enhanced} Conversation and XAI Usage}\label{sec-xai-usage}
% \glcomment{Up to now, no idea what is the difference brought by personalization}
%\glcomment{Provide a clear analysis of why there is no significant difference between control and PCXAI (R3) - shall we mention it here or discussion? Now I put more content in discussion}
To compare how {enhanced} conversation {(\ie adaptive steering for evaluative decision support and more flexible conversational interactions with LLM agents)} affects user interaction with the conversational interface, we analyzed the usage of the XAI methods.
% the chat journeys of users and explored their usage of the XAI methods. ~\glcomment{As our chat journey is incomplete. I think it would be better to not mention chat journey in our paper.}
To compare the usage of each XAI method, we conducted a Kruskal-Wallis H-test for total usage per participant. 
% (results are shown in Table~\ref{tab:personalization}).
Across all five XAI methods, 
no significant differences in usage frequency were found between the \chatxai{} and \chatpersonalized{} conditions. 
The most obvious difference is that participants in the  \chatxai{} and \chatpersonalized{} conditions used PDP method significantly more frequently: \chatxai{}($M=13.5$), \chatpersonalized{}($M=14.1$), \chatagent{}($M=3.6$). 
Meanwhile, participants in the \chatagent{} condition showed significantly more usage of WhatIF, MACE, and SHAP methods than the \chatxai{} and \chatpersonalized{} conditions.
% The most obvious difference is that participants in the \chatpersonalized{} condition tend to obtain SHAP responses more often (on average, around once more per participant). 
The reason for such difference in the usage of XAI methods can be caused by the design of the rule-based conversational agent in the \chatxai{} and \chatpersonalized{} conditions. 
In the rule-based conversation agents, all messages are pre-defined, and users see them in a fixed order. 
Such fixed order may have biased user selection of the XAI responses. %\ug{Add a line about the order of the different XAI methods seen in the two conversational XAI conditions.} \glcomment{I did not conduct such analysis, as decision tree are missing (bug) and PDP are frequently used (bias)}
In comparison, the hint questions are randomized in condition  \chatagent{}, and users can also use the free text input to ask anything they prefer. As a result, participants in the \chatagent{} condition may have more flexible access to explore personalized information needs.
% We provide a pre-defined mode of user queries/responses which may bias user selection of the XAI responses.\glcomment{Any better explanation? I'm thinking about whether it will be recognized as a `robot' and then impact user selection.}
 
% To explore how the XAI interface affects user decision criteria, we conducted a Kruskal-Wallis H-test for \textit{Feature Switch} \gladd{(\ie the number of different features in user initial decision making and final decision making)}
% % \glcomment{I found this is the only use of feature switch in our paper, we can delete the mention of feature switch in the variables part \ug{Agree!}}
% %\ug{add a brief explanation for this?} 
% in the \chatxai{}, \chatpersonalized{}, \chatagent{} conditions. 
% The difference was found to be non-significant (\revise{$H = 0.64$, $p=.733$}). 
% Thus, users did not demonstrate a greater tendency to alter their decision criteria after interacting with the {evaluative conversational XAI interface or conversational XAI interface powered by LLM agents}. 
% \glcomment{We can consider deleting the analysis for personalization. Due to a bug in recording the XAI usage, we do not have complete records of user sequential XAI usage (conversation op sequence). I only have access to total usage per task)} \ug{Oh that's a pity! We can leave this as it is nonetheless; total usage is still useful to know even without the sequences of actions.}

% \glcomment{Compare with Feature Switch}

% What we can check:
% \begin{itemize}
%     \item whether users obtained more explanations to understand their initial top-$3$ features~\glcomment{It can be limited, as some XAI methods do not require human input.}
%     \item whether users increased their usage of conversation
% \end{itemize}


% \begin{table}[htbp]
% 	\centering
% 	\caption{Kruskal-Wallis H-test results for XAI usages on \chatxai{} and \chatpersonalized{}. }
% 	\label{tab:personalization}%
%         % \scalebox{0.95}{
% 	\begin{tabular}{c | c c | c  c }
% 	    \hline
%             \textbf{XAI Method}& $H$& $p$& $M \pm SD$ (\chatxai{})& $M \pm SD$ (\chatpersonalized{})\\
%             \hline
%             \hline
%             \textbf{PDP}& 0.09& .769& 13.5 $\pm$ 7.3& \textbf{14.1 $\pm$ 8.5} \\
%             \textbf{SHAP}& 3.12& .077& 6.7 $\pm$ 3.7& \textbf{7.8 $\pm$ 3.3}\\
%             \textbf{MACE}& 0.06& .801& 1.8 $\pm$ 1.9& 1.8 $\pm$ 1.9\\
%             \textbf{Decision Tree}& 0.06& .801& 2.8 $\pm$ 3.0& \textbf{3.1 $\pm$ 3.3}\\
%             \textbf{What-If}& 0.26& .613& \textbf{4.1 $\pm$ 4.2}& 3.6 $\pm$ 3.4\\
% 	    \hline
% 	\end{tabular}
%     % }%
% \end{table}%


% \subsubsection{Further Analysis of XAI Usage} 
% \glcomment{Due to the bias concern, we do not visualize how the XAI usage patterns. The usage of PDP may get biased due to the design of our rule-based conversational agent.} 
%As the frequent usage of the PDP XAI method in condition \chatxai{} and \chatpersonalized{} may be due to potential bias caused by the conversational agent, we only considered 
To obtain further insights, we explored the user conversation history in the \chatagent{} condition. % for further analysis. 
Among all 61 users in  \chatagent{} , 1,946 user queries are asked in total. Among them, around $40\%$ are based on the hint questions (5 questions we provide to trigger XAI responses, see Table~\ref{tab:xai_conversation}). 
% Among all 61 users in the\chatagent{} condition, 1,946 user queries are asked in total. Among them, around $40\%$ are based on the hint questions (5 questions were provided to trigger XAI responses, see Table~\ref{tab:xai_conversation}). 
The valid user queries mainly consist of three types of intent: user queries to obtain XAI responses (\eg hint questions and some similar questions), greetings (\eg ``Hi'', ``Thank you''), and opinion-seeking queries to the conversational agent (\eg ``Do you think the loan application is creditworthy?''). %Besides them, 
When meaningless user queries are fired (such as gibberish, random strings or something irrelevant to our task context), the LLM agent-based conversational interface can handle them properly (\eg ``I do not understand this. Please check information related to the current task.'').
% It shows that users in condition \chatagent{} did create some questions on themselves to address their information needs. 
To visualize the dynamics of user information needs along with exploring conversation, we adopted the Sankey diagram (Figure~\ref{fig-sankey}) to show the dynamic flow of XAI usage. 
Only a few participants in the \chatagent{} condition asked for more than three XAI responses in each task, so we only considered the first three usages of XAI methods. 
As we can see, after using one XAI method, participants tend to use a different XAI method in the next step, which indicates that most participants explored diverse information needs in the LLM condition \chatagent{}.
%\glcomment{Is there any other meaningful take-away message from the Sankey diagram?}
% \glcomment{Another analysis can be user questions in LLM Agent. What questions going beyond hint questions are used? I also see some meaningless queries like ``Hi''. Add that part to appendix}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/sankey_new.png}
    % \includesvg[scale=0.2]{figures/sankey_new.svg}
    \caption{Illustration of the XAI usage used in our study. This Sankey diagram describes the sequence of interactions with XAI methods by users in the  \chatagent{} experimental condition.}%~\glcomment{Is it fine? Any suggestion to make it better}}
    \label{fig-sankey}
    \Description{{A sankey diagram visualizing the flow of user usage of explainers in the first three steps.}}
\end{figure}
